TinyRadarNN: Combining Spatial and Temporal Convolutional Neural Networks for Embedded Gesture Recognition with Short Range Radars

This work proposes a low-power high-accuracy embedded hand-gesture recognition algorithm targeting battery-operated wearable devices using low power short-range RADAR sensors. A 2D Convolutional Neural Network (CNN) using range frequency Doppler features is combined with a Temporal Convolutional Neural Network (TCN) for time sequence prediction. The final algorithm has a model size of only 46 thousand parameters, yielding a memory footprint of only 92 KB. Two datasets containing 11 challenging hand gestures performed by 26 different people have been recorded containing a total of 20,210 gesture instances. On the 11 hand gesture dataset, accuracies of 86.6% (26 users) and 92.4% (single user) have been achieved, which are comparable to the state-of-the-art, which achieves 87% (10 users) and 94% (single user), while using a TCN-based network that is 7500x smaller than the state-of-the-art. Furthermore, the gesture recognition classifier has been implemented on a Parallel Ultra-Low Power Processor, demonstrating that real-time prediction is feasible with only 21 mW of power consumption for the full TCN sequence prediction network, while a system-level power consumption of less than 100 mW is achieved. We provide open-source access to all the code and data collected and used in this work on tinyradar.ethz.ch.

==> src/summaryOfDifferencesSRR.tex <==
To whom it may concern,
the manuscript entitles "TinyRadarNN: Combining Spatial and Temporal Convolutional Neural Networks for Embedded Gesture Recognition with Short Range Radars" is an extension of our IEEE Sensors 2019 Conference paper "Low Power Embedded Gesture Recognition Using Novel Short-Range Radar Sensors". 

The extension significantly contains new results, ideas and innovations that advance the state-of-the-art in embedded temporal modelling of RADAR. The additions are summarized as follows.
\begin{itemize}
    \item Tuning and evaluation of the network design and pre-processing methods.
    In the original paper, these were not discussed at all. The proposed paper gives an in-depth understanding and study of the impact each part of the network and pre-processing steps has on the final prediction's quality.
    \item Comparison of temporal modelling approaches.
    The extension also includes comparisons between an LSTM-based approach of modelling temporal evolution and a TCN-based approach of modelling.
\end{itemize}
We firmly believe that the novel contributions make up around 50\% of the manuscript.

This paper is intended for potential inclusion in the IEEE Transactions on Pattern Analysis and Machine Intelligence. As the paper contains in-depth evaluations of algorithms for temporal modelling of RADAR data in an embedded setting and an open-source dataset of hand gesture recordings made with a RADAR, we believe it is interesting for the TPAMI audience concerned with machine learning applications for embedded systems. 

Thank you for your considerations and best regards,
Moritz Scherer, Michele Magno, Jonas Erb, Philipp Mayer, Manuel Eggimann and Luca Benini
